Co$^2$L: Contrastive Continual Learning

Recent breakthroughs in self-supervised learning show that such algorithms learn visual representations that can be transferred better to unseen tasks than joint-training methods relying on task-specific supervision. In this paper, we found that the similar holds in the continual learning con-text: contrastively learned representations are more robust against the catastrophic forgetting than jointly trained representations. Based on this novel observation, we propose a rehearsal-based continual learning algorithm that focuses on continually learning and maintaining transferable representations. More specifically, the proposed scheme (1) learns representations using the contrastive learning objective, and (2) preserves learned representations using a self-supervised distillation step. We conduct extensive experimental validations under popular benchmark image classification datasets, where our method sets the new state-of-the-art performance.

==> algorithm/buffer.tex <==

\begin{algorithm}[H]
\caption{Buffer manage algorithm}
\label{alg:buffer}
\begin{algorithmic}[1]

\STATE \textbf{Input}: Buffer size $M$, buffer $\mathcal{M}:=\{(x_i, y_i)\}^M_{i=1}$, a set of current $t$ task samples $\mathcal{D}_t$, a set of disjoint class sets so far $\{\mathcal{C}_k\}^t_{k=1}$.

\STATE TBD
\end{algorithmic}

\end{algorithm}


==> arxiv_Contrastive Continual Learning/Background/base.tex <==
\label{section:background}
In this section, we formalize the considered continual learning setup and briefly describe a recently proposed supervised contrastive learning scheme \cite{khosla20} that will be used as the main framework for designing Co$^2$L (Section~\ref{section:method}).
% {\color{blue}the latter will be used in the sanity check experiment (Section~\ref{subsection:observation}) and will be helpful in describing Co$^2$L (Section~\ref{section:method}).}
\input{Background/problem_fomulation}
\input{figures_tex/submethods}
\input{Background/contrastive_representation_learning}

==> arxiv_Contrastive Continual Learning/Background/contrastive_representation_learning.tex <==
\subsection{Preliminaries: Contrastive Learning}
We now describe the SupCon (Supervised Contrastive learning) algorithm, proposed by \cite{khosla20}. Suppose that the classification model can be decomposed into two components 
\begin{align}
    \varphi_\theta = \mathbf{w} \circ f_{\vartheta}
\end{align}
% $$\varphi_\theta = \mathbf{w} \circ f_{\vartheta}$$
with parameter pairs $\theta = (\vartheta,\mathbf{w})$, where $\mathbf{w}(\cdot)$ is the linear classifier and $f_{\vartheta}(\cdot)$ is the representation. Without training $\mathbf{w}$, SupCon directly trains $f_{\vartheta}$ as follows: Given a batch of $N$ training samples $\{(\mathbf{x}_i,y_i)\}_{i=1}^N$, SupCon first generates an augmented batch $\{(\tilde{\mathbf{x}}_i,\tilde{y}_i)\}_{i=1}^{2N}$ by making a two randomly augmented versions of $\mathbf{x}_k$ as $\tilde{\mathbf{x}}_{2k}, \tilde{\mathbf{x}}_{2k-1}$, with $\tilde{y}_{2k} = \tilde{y}_{2k-1} = y_k$. The samples in the augmented batch are mapped to a unit $d$-dimensional Euclidean sphere as
\begin{align}
    \mathbf{z}_i = (g \circ f)_{\psi}(\tilde{\mathbf{x}}_i),
\end{align}
where $g = g_{\phi}$ denotes the projection map parametrized by $\phi$, and $\psi$ denotes the concatenation of $\vartheta$ and $\phi$. Now, the feature map $(g \circ f)_{\psi}$ is trained to minimize the supervised contrastive loss
\begin{align}
    \mathcal{L}^{\text{sup}} = \sum_{i = 1}^{2N} \frac{-1}{|\mathfrak{p}_i|}\sum_{j \in \mathfrak{p}_i} \log \left(\frac{\exp(\mathbf{z}_i \cdot \mathbf{z}_j / \tau)}{\sum_{k \ne i}\exp(\mathbf{z}_i \cdot \mathbf{z}_k / \tau)}\right), \label{eqn:supcon}
\end{align}
where $\tau > 0$ is some temperature hyperparameter and $\mathfrak{p}_i$ is the index set of positive samples with respect to the anchor $\tilde{\mathbf{x}}_i$, defined as
\begin{align}
    \mathfrak{p}_i = \big\{j \in \{1,\ldots,2N\} ~\big|~\:j \ne i,\: y_j = y_i\big\}.
\end{align}
In other words, the sample in $\mathfrak{p}_i$ is either the other augmentation of the unaugmented version of $\tilde{\mathbf{x}}_i$, or one of the other augmented samples having the same label.

%Contrastive representation learning scheme aims to train an encoder that distinguish semantically similar images from others in embedding space. Specifically, the encoder $f_\theta$ attempts to make embeddings of the set of positive samples ${\{x_{+}\}}$ to be similar and the set of negative samples ${\{x_{-}\}}$ to be dissimilar with respect to the query $x$. 

%\textbf{Self-Supervised Contrastive Loss} 
%The idea of self-supervised contrastive representation learning is constructing positive/negative sets by leveraging pretext task without actual class labels. One of the most popular approach of this line of work is simple contrastive learning (\textit{SimCLR}) which uses a pair of augmented views from an image as a positives and other augmented views from different images as negatives. Let $\bar{x}_{i}:=h(x_i)$ be an augmentation of image $x_i$ where $h$ be an independently drawn augmentation from predefined family $\mathcal{H}$. The $i\in I \equiv \{1,...,2N\}$ is an arbitrary sample index of independently augmented $N$ pairs of images, and $j(i)$ is the index of augmented counterpart of image ${x_i}$.
% $x_i:=T^{1}(x)$ and $x_{j(i)}:=T^{2}(x)$ be a pair of augmented image $x$ from the independent augmentations, $T^{(1)}, T^{(2)} \sim \mathcal{T}$, where $\mathcal{T}$ is a predefined transformation family. The augmented images are encoded from the encoder $f_{\theta}$ and then projected and normalized by the projection layer $g_{\phi}$, i.e., $\mathbf{z_i} = g_{\phi}(f_{\theta}(\bar{x}_i))$. In the end, the SimCLR objective is defined as follows:

%\begin{equation}
%\label{eqn:simclr}
%    \mathcal{L}^{\text {self}}=-\sum_{i \in I} \log \frac{\exp \left(\mathbf{z}_{i} \cdot \mathbf{z}_{j(i)} / \tau\right)}{\sum_{k \in I \setminus \{i\}} \exp \left(\mathbf{z}_{i} \cdot \mathbf{z}_{k} / \tau\right)}
%\end{equation}
%where $\tau$ is a temperature hyperparameter. 

%\textbf{Supervised Contrastive Loss}
%\citet{khosla20} extend eq.~\eqref{eqn:simclr} when class labels are available and show it outperforms supervised learning of joint training schemes. Supervised contrastive loss considers all augmented samples of the same class to belong to a positive set. Specifically, let $P(i)$ be a set of indices of samples with the same label as $y_i$, and let $p \in P(i)$ be an arbitrary sample index in $P(i)$. In the end, the supervised contrastive loss is defined as follows:

%\begin{equation}
%\label{eqn:supcon}
%    \mathcal{L}^{\text {sup }}=\sum_{i \in I} \frac{-1}{|P(i)|} \sum_{p \in P(i)} \log \frac{\exp \left(\mathbf{z}_{i} \cdot \mathbf{z}_{p} / \tau\right)}{\sum_{k\in I \setminus \{i\}} \exp \left(\mathbf{z}_{i} \cdot \mathbf{z}_{k} / \tau\right)}
%\end{equation}

==> arxiv_Contrastive Continual Learning/Background/problem_fomulation.tex <==
\subsection{Problem Setup: Continual Learning}
\label{subsection:problem-setup}

We consider three popular scenarios of continual learning as categorized by \cite{vandeven2019three}: task-incremental learning (Task-IL), domain-incremental learning (Domain-IL), and class-incremental learning (Class-IL).

Formally, the learner is trained on a sequence of tasks indexed by $t \in \{1,2,\ldots,T\}$. For each task, we suppose that there is a task-specific class set $C_t$. For Task-IL and Class-IL, $\{C_t\}_{t=1}^T$ are assumed to be disjoint, \ie,
\begin{align}
    t \ne t' \Rightarrow C_t \cap C_{t'} = \emptyset, \qquad \text{(Task/Class-IL).}
\end{align}
For Domain-IL, $C_t$ remains the same throughout the tasks:
\begin{align}
    C_1 = C_2 = \cdots = C_T, \qquad \text{(Domain-IL)}.
\end{align}
During each task, $n_t$ copies of training input-label pairs are independently drawn from some task-specific distribution, \ie, $\{(\mathbf{x}_i,y_i)\}_{i=1}^{n_t} \sim D_t$.
Here, $\mathbf{x}$ denotes the input image, and $y_i \in C_t$ denotes the class label belonging to the task-specific class set. For Task-IL, the learned models are assumed to have access to the task label $t$ during the test phase; the goal is to find a predictor $\varphi_{\theta}(\mathbf{x},t)$ parameterized by $\theta$ such that
\begin{align}
    \mathcal{L}(\theta) := \sum_{t=1}^T \mathbb{E}_{D_t}[\ell(y,\varphi_\theta(x,t))], \qquad \text{(Task-IL)}
\end{align}
is minimized for some loss function $\ell(\cdot,\cdot)$. For Domain-IL and Class-IL, the model cannot access the task label during the test phase; the goal is to find a predictor $\varphi_{\theta}(\mathbf{x})$ minimizing
\begin{align}
    \mathcal{L}(\theta) = \sum_{t=1}^T \mathbb{E}_{D_t}[\ell(y,\varphi_\theta(x))], \quad \text{(Domain/Class-IL).}
\end{align}


%Continual lifelong learning is a research area that aims to learn new knowledge without compromising the performance achieved on the past tasks under the settings where the access to past samples is limited.  Most of related studies follow class incremental learning settings where a model is trained on disjoint sets of class samples in a sequential manner. Formally, a model is trained on a given samples $\{(x_i, y_i)\} \sim D_t$ where $D_t$ is a distribution of task $t\in\{1,...,T\}$. For each task, the set of classes of $\{(x_i, y_i)\} \sim D_t$, denoted by $C_t$, is mutually exclusive to $C_s$ for $t \neq s$. At the end of training, the trained model is evaluated on the test samples from all classes observed so far, i.e., $\bigcap_i{C_i}$. Other lines of studies in continual learning extend the scope of such settings to involve domain shifts, so-called domain incremental learning. In this setting, the set of classes $C_t$ is equal for all tasks, but the domains of tasks are quite different each other. 

==> arxiv_Contrastive Continual Learning/Experiment/base.tex <==



\label{section:experiment}
\subsection{Experimental Setup}
\label{subsection:exp_setup}
\noindent\textbf{Learning scenarios and datasets.}
Following \cite{vandeven2019three}, we conduct continual learning experiments on Task Incremental Learning (Task-IL), Class Incremental Learning (Class-IL) and Domain Incremental Learning (Domain-IL) scenarios. 
We conduct experiments on Seq-CIFAR-10 and Seq-Tiny-ImageNet for Task-IL and Class-IL scenarios and R-MNIST for Domain-IL scenario. 
\textbf{Seq-CIFAR-10} is the set of splits (tasks) of the CIFAR-10 \cite{krizhevsky2009learning} dataset. We split the CIFAR-10 dataset into five separate sample sets, and each sample set consists of two classes. Similarly, \textbf{Seq-Tiny-ImageNet} is built from Tiny-ImageNet \cite{Le2015TinyIV} by splitting 200 class samples into 10 disjoint sets of samples, each consisting of 20 classes.
Seq-CIFAR-10 and Seq-Tiny-ImageNet split are given in the same order across different runs, as in \cite{buzzega20}.
We conduct experiments on \textbf{R-MNIST} \cite{lopezpaz17} for Domain-IL experiments. 
For Domain-IL scenario, R-MNIST is constructed by rotating the original MNIST \cite{lecun98} images by a random degree in the range of [0, $\pi$). R-MNIST consists of 20 tasks, corresponding to 20 uniformly randomly chosen degrees.
We note that we treat samples from different domains with the same digit class as different classes while applying asymmetric supervised contrastive loss. 

% \textbf{Datasets.}
% \textbf{Seq-CIFAR-10} is the set of splits(tasks) of CIFAR-10 dataset. We split the CIFAR-10 dataset into five separate sample sets, and the class composition of each set consists of two classes that do not overlap each other. Similarly, \textbf{Seq-Tiny-ImageNet} is built from Tiny-ImageNet by splitting 200 class samples into 10 disjoint set of samples. 


\vspace{0.2em}
\noindent\textbf{Training.}
We compare our contrastive continual learning algorithm with rehearsal-based continual learning baselines: ER \cite{riemer19}, iCaRL \cite{Rebuffi17}, GEM \cite{lopezpaz17}, A-GEM \cite{chaudhry19}, FDR \cite{benjamin19}, GSS \cite{aljundi19}, HAL \cite{chaudhry20}, DER \cite{buzzega20}, and DER++ \cite{buzzega20}. We train ResNet-18 \cite{He2015} on Seq-CIFAR-10 and Tiny-ImageNet, and a simple network with convolution layers on R-MNIST. 
For all baselines, we report performance given in \cite{buzzega20} of buffer size 200 and 500 except for R-MNIST since we choose a different architecture. 
% We follow the best hyperparameters introduced in \cite{buzzega20} for those baselines. 
% We choose ResNet-18 \cite{He2015} as a base architecture for Seq-CIFAR-10 and Seq-Tiny-ImageNet, and a simple convolutional neural network (2 Conv + fc) for R-MNIST. 
More training details are provided in the supplementary material.

% \textbf{Training Details.}
% We choose ResNet-18 as a base architecture for Seq-CIFAR-10 and Seq-Tiny-ImageNet, and a simple convolutional neural network (2 Conv + fc) for R-MNIST. Details of architecture are provided in supplementary material.   
% For all datasets, we apply random crop and horizontal flip for baselines and \textit{RandomResizedCrop}, \textit{ColorJitter}, \textit{RandomGrayScale} and horizontal flip for ours, following the data augmentation scheme introduced in \citet{khosla20}. 
% For all baselines, we use hyperparameters introduced in \citet{buzzega20} since they already provide hyperparameter for reproducing best results by performing a grid-search. 
% In our case, we simply use all same learning rates and scheduling, training epochs, batch size, and temperature parameters for supervised contrastive loss (eq.~\eqref{eqn:supcon} and instance-wise distillation loss. 
% We train our models using Stochastic Gradient Descent (SGD) optimizer with weight decay and momentum. 

\vspace{0.2em}
\noindent\textbf{Evaluation protocol for Co$^2$L.}
As Co$^2$L is a representation learning scheme and not a joint representation-classifier training, we need to train a classifier additionally. For a fair comparison, we train a classifier using only the last task samples and buffered samples on top of the frozen representations learned by Co$^2$L. To avoid the class-imbalance problems, we train a linear classifier with a class balanced sampling strategy, where first a class is selected uniformly from the set of classes, and then an instance from that class is subsequently uniformly sampled. 
% Specifically, the probability $p_j$ of sampling a data point from class $j$ is given by $p_j = n_j / {\sum_{c \in \mathcal{C}} n_c}$
% where $n_c$ denotes the number of samples of class $c$. 
We train a linear classifier for 100 epochs for all experiments, and we report classification test accuracy on this classifier.




% As described in Section~\ref{section:method}, it is non-trivial to train a linear classifier upon contrastively learned representation in continual learning setup; it is necessary to use at least a small portion of past samples to train a classifier, which is the one of main reasons we use a replay buffer. 
% Since currently available past samples might be too small, a na\"{i}vely trained classifier would severely suffer from class-imbalance problems. Hence, we train a linear classifier with a class balanced sampling strategy on the union of last task samples and buffered samples. Specifically, the probability $p_j$ of sampling a data point from class $j$ is given by $p_j = n_j / {\sum^{\mathcal{C}} n_c}$
% where $n_c$ denotes the number of samples of class $c$. We train a linear classifier for 100 epochs for all experiments, and we report classification test accuracy on this classifier.

\input{Experiment/table/main_table}

\input{Observation/observation}


\vspace{0.2em}
\noindent\textbf{Superiority of Co$^2$L over baselines.}
%\label{subsection:main-results}
As shown in Table~\ref{main-table}, our contrastive continual learning algorithm consistently outperforms all baselines in various scenarios, datasets, and memory sizes. 
Such results indicate that our algorithm successfully learns and preserves representations useful for future learning, and thus it significantly mitigates catastrophic forgetting. 
Moreover, such consistent gains over all comparisons show that our scheme is not limited to certain incremental learning scenarios.
In what follows, we provide a more detailed analysis of our algorithm.

\subsection{Ablation Studies}
\label{subsection:ablation}


\noindent\textbf{Effectiveness of IRD.}
To verify the effectiveness of IRD, we perform an ablation experiment with the class-IL setup on the Seq-CIFAR-10 dataset (identical to the setup in Section~\ref{subsection:observation}), with three additional variants of Co$^2$L. \textit{(a) without buffer and IRD:} We optimize using only the SupCon loss (eq.~\ref{eqn:supcon}); the symmetric version is identical to the asymmetric one since we do not use a replay buffer. \textit{(b) with IRD only:} We use both (symmetric) SupCon loss and IRD loss. \textit{(c) with replay buffer only:} We optimize the asymmetric SupCon loss (eq.~\ref{eqn:supcon_asym}) without an IRD loss. Note that while we do not use buffered samples to learn representations for (a,b), we still need buffered samples to train the downstream linear classifier; for (a,b), we use 200 auxiliary buffered samples to train the classifier (as in (c) and Co$^2$L).

%To verify the effectiveness of IRD, we simply train our model on Seq-CIFAR-10 dataset in the same setting of Section~\ref{subsection:main-results} by optimizing asymmetric supervised contrastive loss (eq.~\ref{eqn:supcon_asym}) \textit{(a) without buffer and IRD}, \textit{(b) with IRD only}, \textit{(c) with replay buffer only} and \textit{(d) with our proposed method}. Note that the samples used to train linear classifiers are identical between (a) and (c) and between (b) and (d) for fair comparison.

As shown in Table~\ref{ablation-table}, IRD brings a significant performance gain, with or without the replay buffer. With the replay buffer (rows (c,d)), we observe a 22.40\% relative improvement; without the replay buffer (rows (a,b)), there is a 10.59\% relative improvement. The former is noticeably larger than the latter; we suspect that maintaining the similarity structure of buffered samples (along with current task samples) is essential in preserving learned representations.
%As shown in Table~\ref{ablation-table}, the performance significantly increases with 22.40\% relative improvements when the replay strategy comes with IRD (rows (c) and (d)), which indicates that applying relation distillation is the main source of our greatness.  
%IRD also improves the utility on buffered samples: the relative improvement 22.40\% between (d) and (c) is much larger than that 10.59\% between (b) and (a). 
%Surprisingly, our relation distillation solely gives performance improvement without buffered samples while learning representations (row (c)). This indicates that distilling relation only with current task samples also can help to preserve learned representations presumably because contrastively learned representations are useful enough to perform unseen tasks. This also shows that IRD can enjoy the benefits of distillation relying on the relation between any samples not the exact representations itself. 

% We also note that the performance boost from using the replay buffer--and thus asymmetric SupCon loss--becomes relatively insignificant without IRD (rows (a,c)).


% This highlights the complementary role of IRD and asymmetric SupCon in terms of using buffered samples. As shown in Figure~\ref{fig:ird_asym}, ~~.
% In contrast, asymmetric SupCon loss is designed to learn representations continually without hurting learned ones on purpose, which we will observe in the next ablation study on asymmetric supervised contrastive loss. 

% IRD 없이는? 퍼포먼스 부스트가 거의 없어  -> IRD는 버퍼가 있는 환경에서 (혹은 그렇지 않은 환경이더라도) (orignal과 비교했을때) asymmetricity로 인해 발생하는 부작용을 (b,d)를 통해 + figure 3를 통해 모든 memory setup에서 잘 해줄거란걸 알 수 있어. -> 그럼 결국 asymmetric이 구리단거야? -> 아니야. asymmetricity는 IRD 없이는 부족해보이지만 앞선 method 섹션에서 다룬 우리의 직관대로 나름의 긍정적 이익이 있어. 다음 섹션을 보자!
We also note that IRD seems to complement the asymmetric SupCon in terms of using buffered samples, leading to a performance boost. To verify this, we consider a synthetic \textit{infinite-buffer} class-IL scenario: all past samples are available throught the training. Under this setup, we train a model with $\mathcal{L}^{\text {sup }}$ and another with $\mathcal{L}^{\text {sup }}_{\text{asym}}$ on Seq-CIFAR-10. As shown in Figure~\ref{fig:ird_asym}, asymmetric SupCon performs relatively poor without using IRD; under this class-balanced setup, not using past task samples as positive pairs only restricts learning. With increasing IRD power, however, the performance gap closes, indicating that IRD complements asymmetric SupCon by helping fully utilize the buffered samples. 
Such trend is also aligned with the results in Table~\ref{ablation-table}; the performance boost from buffered samples--and thus asymmetric SupCon loss--is relatively small without using IRD. This, however, does not necessarily imply that asymmetricity does not bring any benefit, as we will observe in the following ablation study on asymmetric SupCon.


% We also note that the performance boost from using the replay buffer---and thus asymmetric SupCon loss---becomes relatively insignificant without IRD (rows (a,c)). This does not necessarily imply that asymmetricity does not bring any benefit, as we will observe in the ablation experiment on Asymmetric SupCon (which will follow shortly).

% We also verify that IRD can preserve learned representations though our main learning objective uses only current task samples as positive anchors. We consider synthetic ideal class-IL scenario that all past samples are available both on representation learning and linear classifier training. Under this setting, we train models one with $\mathcal{L}^{\text {sup }}$ and the other with $\mathcal{L}^{\text {sup }}_{\text{asym}}$ on Seq-CIFAR-10. As shown in Figure~\ref{fig:ird_asym}, Representations learned on $\mathcal{L}^{\text {sup }}_{\text{asym}}$ are not preserved well without IRD. With increasing IRD power, however, the performance gap between learning schemes are closing, which indicates IRD successfully preserves learned representations without using past samples as positive anchors in contrastive objective. 


% \label{subsection:asym-supcon}
\input{Experiment/table/ablation}
\input{figures_tex/ird_asym}



\vspace{0.2em}
\noindent\textbf{Effectiveness of asymmetric supervised contrastive loss.} 
To verify the effectiveness of asymmetric supervised contrastive loss, we compare two contrastive learning losses, the original SupCon and the asymmetric SupCon, as variants of Co$^2$L  with the identical settings of Section~\ref{subsection:observation}.
As shown in Table~\ref{ablation-table-supcon}, asymmetric SupCon consistently provides gains over all counterparts with the original SupCon.
% To verify the effectiveness of asymmetric supervised contrastive loss (Section~\ref{subsection:asymsup}), we compare $\mathcal{L}^{\text{sup}}_{\text{asym}}$ with $\mathcal{L}^{\text{sup}}$.
 
We also compare the visualizations of encoders' outputs of buffered and entire training samples of the Seq-CIFAR-10 dataset where the encoders are trained in the ablation experiments of Table~\ref{ablation-table-supcon}.
As illustrated in Figure~\ref{fig:ablation_asym_sup}, buffered samples' features trained with original SupCon are close to the same class samples while ones with asymmetric SupCon are well-spread. Since the buffered samples with asymmetric SupCon better represents the entire class sample population, representations trained on asymmetric SupCon show better task performance with linear classifiers. 
Such qualitative results are also well aligned with the motivation of asymmetric SupCon mentioned in Section~\ref{subsection:asymsup} and provide the benefits of asymmetricity. 

% As illustrated in Section \ref{subsection:asymsup}, supervised contrastive loss on a few observable samples can change feature spaces dramatically while features of those get close each other by being used as positive anchors/pairs. 
% We qualitatively observe such phenomenon from visualization of encoder's output of buffered samples and entire samples. 
% In Figure~\ref{fig:ablation_asym_sup}, the available samples' features (colored marks) well spread the entire region of features of all observed samples (gray marks) when $\mathcal{L}^{\text{sup}}_{\text{asym}}$ is used. It can be interpreted that the classifier learning performance is higher even in class imbalance situations because the representation regions covered by the available samples are more equally well separated by class in case of using $\mathcal{L}^{\text{sup}}_{\text{asym}}$.
% the colored marks visualize features of buffered samples and the gray ones represent features from all entire samples observed so far. From this visualization, the area that buffered samples cover is much larger and self-contained when the asymmetric form of supervised contrastive loss is applied. 

% well aligned, as we expected...

% We investigate how asymmetric form of supervised contrastive loss (eq.~\eqref{eqn:supcon_asym}) improves performance in quantitative and qualitative analysis. We simply replace $\mathcal{L}^{\text{sup}}_{\text{asym}}$ with $\mathcal{L}^{\text{sup}}$ and compare the performance on Seq-CIFAR-10, and Seq-Tiny-ImageNet. As shown in Table \ref{ablation-table-supcon}, the performance significantly drops over all counterparts.

\input{Experiment/table/ablation_supcon}
\input{figures_tex/asym_tiled}










% \subsection{Effect of Distillation Temperatures}
% We simply apply IRD to distill past relation to current one with temperature parameters $\tau^{\ast}$ and $\tau$. Meanwhile, one can extend such temperature parameters to assign different temperature scaling for each instance-wise relation since the importance of relation defined on a sample may different within batch samples. 
% Specifically, the instance-wise relation of observed samples at the end of the $t$ task training should be more consolidated that the one of samples to be learned. We thus separate batch samples into current task sample group and past tasks sample group, and assign different temperature values for each group as $\tau^{\ast}_{\text{past}}, \tau^{\ast}_{\text{current}}, \tau_{\text{past}}$ and $\tau_{\text{current}}$. 





==> arxiv_Contrastive Continual Learning/Experiment/table/ablation.tex <==
\begin{table}[t]
\setlength{\tabcolsep}{0.2cm}
\centering

% \vskip 0.15in
\begin{center}
\begin{small}
\begin{tabular}{lccc}
\toprule
& Buffer Size & IRD & Accuracy(\%) \\
\midrule
(a) w/o buffer and IRD & 0 & \color{red}\xmark  & 53.25\stdv{1.70} \\
(b) w/ IRD only & 0 & \color{green}\cmark & 58.89\stdv{2.61} \\
(c) w/ buffer only & 200 & \color{red}\xmark & 53.57\stdv{1.03} \\
(d) Co$^2$L(ours) & 200 & \color{green}\cmark & \textbf{65.57\stdv{1.37}} \\
\bottomrule
\end{tabular}


\end{small}
\end{center}
\caption{Ablation study of Instance-wise Relation Distillation (IRD). We train our model on Seq-CIFAR-10 dataset under class-IL scenario (identical to the setup in Section~\ref{subsection:observation}) with ablated Co$^2$L. IRD brings significant gain with or without replay buffer. All results are averaged over ten independent trials.}
\label{ablation-table}
\end{table}

==> arxiv_Contrastive Continual Learning/Experiment/table/ablation_supcon.tex <==
\begin{table}[t]
\setlength{\tabcolsep}{0.2cm}
\centering
% \vskip 0.15in
\begin{center}
\begin{small}
\resizebox{\columnwidth}{!}{
\begin{tabular}{ccccccccc}
\toprule
&& \multicolumn{2}{c}{ Seq-CIFAR-10 } & & \multicolumn{2}{c}{ Seq-Tiny-ImageNet } & \\
\cmidrule{3-4}  \cmidrule{6-7}
Buffer  && 200 & 500 & & 200 & 500  &\\
\midrule
$\mathcal{L}^{\text{sup}}$ && 60.49\stdv{0.72} & 68.66\stdv{0.68} & & 13.51\stdv{0.48} & 19.68\stdv{0.62} & \\
$\mathcal{L}^{\text{sup}}_{\text{asym}}$ && \textbf{65.57\stdv{1.37}} & \textbf{74.26\stdv{0.77}} & & \textbf{13.88\stdv{0.40}} & \textbf{20.12\stdv{0.42}} & \\

\bottomrule
\end{tabular}
}
\end{small}
\end{center}

\caption{The effectiveness of asymmetric SupCon loss ($\mathcal{L}^{\text{sup}}_{\text{asym}}$) versus the original SupCon loss ($\mathcal{L}^{\text{sup}}$), combining with the IRD loss. All results are averaged over ten independent trials.}
\label{ablation-table-supcon}

\end{table}

==> arxiv_Contrastive Continual Learning/Experiment/table/main_table.tex <==
% \begin{table*}[ht]
% \setlength{\tabcolsep}{0.2cm}
% \centering
% \caption{Classification accuracies for CIFAR-10, ImageNet-30 and DomainNet-20 on rehearse-based baselines and our algorithm. We consider various buffer size and learning scenarios. The best performance marked as bold.}
% \label{main-table}
% % \vskip 0.15in
% \begin{center}
% \begin{small}
% % \begin{sc}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{ccccccccccccccccc}
% \toprule
% Dataset & & \multicolumn{5}{c}{ CIFAR-10 } & & \multicolumn{5}{c}{ ImageNet-30 } & & \multicolumn{3}{c}{ DomainNet-20 } \\\cmidrule{3-7} \cmidrule{9-13} \cmidrule{15-17}
% Buffer & & \multicolumn{2}{c}{ 200 } & & \multicolumn{2}{c}{ 500 } & & \multicolumn{2}{c}{ 200 } & & \multicolumn{2}{c}{ 500 } & & 200 & & 500 \\ \cmidrule{3-4} \cmidrule{6-7} \cmidrule{9-10} \cmidrule{12-13} \cmidrule{15-17}
% Scenario & & Class-IL & Task-IL & & Class-IL & Task-IL & & Class-IL & Task-IL & & Class-IL & Task-IL & & \multicolumn{3}{c}{ Domain-IL } \\
% \midrule
% ER & & & & & & & & & & & & & & & & \\
% MER & & & & & & & & & & & & & & - & & - \\
% GEM & & & & & & & & & & & & & & & & \\
% A-GEM & & & & & & & & & & & & & & & & \\
% iCaRL & & & & & & & & & & & & & & - & & - \\
% FDR & & & & & & & & & & & & & & & & \\
% GSS & & & & & & & & & & & & & & & & \\
% HAL & & & & & & & & & & & & & & & & \\
% DER++ & & & & & & & & & & & & & & & & \\
% \midrule
% Ours & & & & & & & & & & & & & & & & \\
% \bottomrule
% \end{tabular}
% }
% % \end{sc}
% \end{small}
% \end{center}
% \vskip -0.1in
% \end{table*}


\begin{table*}[ht]
\setlength{\tabcolsep}{0.2cm}
\centering
% \vskip 0.15in
\begin{center}
\begin{small}
% \begin{sc}
\resizebox{0.70\textwidth}{!}{
\begin{tabular}{clccccccccccc}
\toprule
\multirow{2}{*}{ Buffer } & Dataset & & \multicolumn{2}{c}{ Seq-CIFAR-10 } & & \multicolumn{2}{c}{ Seq-Tiny-ImageNet } & & R-MNIST & \\
\cmidrule{4-5} \cmidrule{7-8} \cmidrule{10-10}
& Scenario & & Class-IL & Task-IL  & & Class-IL & Task-IL & & Domain-IL & \\
\midrule
\multirow{10}{*}{ 200 } 
& ER \cite{riemer19}
& & 44.79\stdv{1.86} & 91.19\stdv{0.94} 
& & 8.49\stdv{0.16} & 38.17\stdv{2.00} 
& & 93.53\stdv{1.15} &  \\
& GEM \cite{lopezpaz17}
& & 25.54\stdv{0.76} & 90.44\stdv{0.94} 
& & -  & - 
& & 89.86\stdv{1.23} & \\
& A-GEM \cite{chaudhry19}
& & 20.04\stdv{0.34} & 83.88\stdv{1.49} 
& & 8.07\stdv{0.08} & 22.77\stdv{0.03} 
& & 89.03\stdv{2.76} & \\
& iCaRL \cite{Rebuffi17}
& & 49.02\stdv{3.20} & 88.99\stdv{2.13} 
& & 7.53\stdv{0.79} & 28.19\stdv{1.47} 
& &  - & \\
& FDR \cite{benjamin19}
& & 30.91\stdv{2.74} & 91.01\stdv{0.68} 
& & 8.70\stdv{0.19} & 40.36\stdv{0.68} 
& & 93.71\stdv{1.51} & \\
& GSS \cite{aljundi19}
& & 39.07\stdv{5.59} & 88.80\stdv{2.89} 
& & - & - 
& & 87.10\stdv{7.23} &\\
& HAL \cite{chaudhry20}
& & 32.36\stdv{2.70} & 82.51\stdv{3.20} 
& & - & - 
& & 89.40\stdv{2.50} & \\
& DER \cite{buzzega20}
& & 61.93\stdv{1.79} & 91.40\stdv{0.92} 
& & 11.87\stdv{0.78} & 40.22\stdv{0.67} 
& & 96.43\stdv{0.59} & \\
& DER++ \cite{buzzega20}
& & 64.88\stdv{1.17} & 91.92\stdv{0.60} 
& & 10.96\stdv{1.17} & 40.87\stdv{1.16} 
& & 95.98\stdv{1.06} & \\
& \textbf{Co$^2$L (ours)} 
& & \textbf{65.57\stdv{1.37}}& \textbf{93.43\stdv{0.78}} 
& & \textbf{13.88\stdv{0.40}} & \textbf{42.37\stdv{0.74}} 
& & \textbf{97.90\stdv{1.92}}& \\
\midrule
\multirow{10}{*}{ 500 } 
& ER \cite{riemer19}
& & 57.74\stdv{0.27} & 93.61\stdv{0.27} 
& & 9.99\stdv{0.29} & 48.64\stdv{0.46} 
& & 94.89\stdv{0.95} &  \\
& GEM \cite{lopezpaz17}
& & 26.20\stdv{1.26} & 92.16\stdv{0.64} 
& & - & -
& & 92.55\stdv{0.85} & \\
& A-GEM \cite{chaudhry19}
& & 22.67\stdv{0.57} & 89.48\stdv{1.45} 
& & 8.06\stdv{0.04} & 25.33\stdv{0.49} 
& & 89.04\stdv{7.01} & \\
& iCaRL \cite{Rebuffi17}
& & 47.55\stdv{3.95} & 88.22\stdv{2.62} 
& & 9.38\stdv{1.53} & 31.55\stdv{3.27} 
& &  - & \\
& FDR \cite{benjamin19}
& & 28.71\stdv{3.23} & 93.29\stdv{0.59} 
& & 10.54\stdv{0.21} & 49.88\stdv{0.71} 
& & 95.48\stdv{0.68} & \\
& GSS \cite{aljundi19}
& & 49.73\stdv{4.78} & 91.02\stdv{1.57} 
& & - & - 
& & 89.38\stdv{3.12} &\\
& HAL \cite{chaudhry20}
& & 41.79\stdv{4.46} & 84.54\stdv{2.36} 
& & - & - 
& & 92.35\stdv0.81 & \\
& DER \cite{buzzega20}
& & 70.51\stdv{1.67} & 93.40\stdv{0.39} 
& & 17.75\stdv{1.14} & 51.78\stdv{0.88} 
& & 97.57\stdv{1.47} & \\
& DER++ \cite{buzzega20}
& & 72.70\stdv{1.36} & 93.88\stdv{0.50} 
& & 19.38\stdv{1.41} & 51.91\stdv{0.68} 
& & 97.54\stdv{0.43} & \\
& \textbf{Co$^2$L (ours)} 
& & \textbf{74.26\stdv{0.77}}& \textbf{95.90\stdv{0.26}} 
& & \textbf{20.12\stdv{0.42}} & \textbf{53.04\stdv{0.69}}
& & \textbf{98.65 \stdv{0.31}}& \\
\bottomrule
\end{tabular}
}


% \end{sc}
\end{small}
\end{center}
\caption{Classification accuracies for Seq-CIFAR-10, Seq-Tiny-ImageNet and R-MNIST on rehearsal-based baselines and our algorithm. We report performance of baslines of Seq-CIFAR-10 and Seq-Tiny-ImageNet from \cite{buzzega20}. ‘-’ indicates experiments unable to run due to compatibility issues (\eg, iCaRL in Domain-IL) or intractable training time (\eg, GEM, HAL or GSS on Tiny ImageNet). All results are averaged over ten independent trials. The best performance marked as bold.
}
\label{main-table}
\vspace{-1em}
\end{table*}

==> arxiv_Contrastive Continual Learning/Method/IRD.tex <==
\subsection{Instance-wise Relation Distillation (IRD) for Contrastive Continual Learning}
\label{subsection:IRD}

While using the contrastive learning objective (eq.~\ref{eqn:supcon_asym}) readily provides a more transferable representation, one may still benefit from having an explicit mechanism to preserve the learned knowledge. Taking the inspiration from \cite{fang20}, we propose an instance-wise relation distillation (IRD); IRD regulates the changes in feature relation between batch samples via self-distillation  (see Figure~\ref{subfig:ird}).
%Chen \etal~\cite{Chen19} pointed out that it is crucial to incentivize the model to preserve learned knowledge in order to prevent catastrophic forgetting since currently acquired representations would be of no use in near future. It is, however, not convincing that contrastive representation learning schemes on the continual learning setup solely regulate the model to preserve learned representations.
%To this end, we propose an instance-wise relation distillation (IRD) which is a self-distillation loss for contrastive continual learning, inspired by \cite{fang20}. 
%IRD regulates the changes in feature relation between batch samples. 
Formally, we define the IRD loss $\mathcal{L}^{\text{IRD}}$ as follows: For each sample $\tilde{\mathbf{x}}_i$ in a batch $\mathcal{B}$, we define the \textit{instance-wise similarity vector}
\begin{align}
\label{eqn:simvec}
    \mathbf{p}\left(\tilde{\mathbf{x}}_{i} ; \psi, \kappa\right)=\left[p_{i, 1},  \ldots, p_{i, i-1}, p_{i, i+1},\ldots,p_{i,2N}\right],
\end{align}
where $p_{i,j}$ denotes the normalized instance-wise similarity
\begin{align}
p_{i,j}&=\frac{\exp \left(\mathbf{z}_{i} \cdot \mathbf{z}_{j} / \kappa\right)}{\sum_{k \neq i}^{2N} \exp \left(\mathbf{z}_{i} \cdot \mathbf{z}_{k} / \kappa\right)}
\end{align}
given the representation parameterized by $\psi$ and the temperature hyperparameter $\kappa$. In other words, the instance-wise similarity vector $\mathbf{p}(\cdot)$ is the normalized similarity of a sample to other samples in the batch.

Roughly, the IRD loss quantifies the discrepancy between the instance-wise similarities of the current representation and the past representation; the past representation is a snapshot of the model at the end of the previous task. Denoting the parameters of the past/current model as $\psi^{\text{past}}$ and $\psi$, the IRD loss is defined as
\begin{align}
\label{eqn:IRD}
    \mathcal{L}^{\text {IRD }}  &=\sum_{i=1}^{2N}-\mathbf{p}\left(\tilde{\mathbf{x}}_{i} ; \psi^{\text{past}}, \kappa^{\ast}\right) \cdot \log \mathbf{p}\left(\tilde{\mathbf{x}}_{i} ; \psi, \kappa\right),
\end{align}
where the logarithms and multiplications on the vectors denote the entrywise logarithms and multiplications. We note that we are using different temperature hyperparameters for the past and current similarity vectors; on the other hand, both $\kappa,\kappa^*$ will remain fixed throughout the tasks.

%Let us denote currently available $N$-sized dataset by $\mathcal{D}$ which is the union of current training set $\mathcal{D}_t$ and the buffer set $\mathcal{M}$ at task $t$. The batch set denoted by $\mathcal{B}$ then consists of augmented views of $\mathcal{D}$ with pre-defined augmentation family $\mathcal{H}$. 
% $\{(\tilde{\mathbf{x}}_i,\tilde{y}_i)\}_{i=1}^{2N}$

%The instance-wise similarity vector $\mathbf{p}(\cdot)$ for an arbitrary augmented view $\tilde{\mathbf{x}}_i \in \mathcal{B}$, trained model weights $\psi$, and temperature hyperparameter $\kappa$ is defined as follows:

% Hence, in the following sections, we'll propose explicitly designed training scheme for contrastive continual learning.
% Based on our observation, it is clear that contrastively learned representation is good at retaining its discriminative power. Under the limitation of classifier re-training procedure on buffered samples, however, the use of buffered samples should be designed differently from the one with the joint training schemes. Namely, continual representation learning should aim to construct representation which is robust itself to forgetting in the absence of any classifier. 
% Meanwhile, most of the recent advances on replay based continual learning come with regulating prediction changes in forms of knowledge distillation or logit matching. Similar to those approaches on joint learning schemes, regulating representation changes through sequential tasks can maintain representations robust to forgetting. 
% Inspired by this simple idea, we propose instance-wise relation distillation (IRD) which is specifically designed for contrastive continual learning. IRD regulates the changes in relationship between batch samples. Let us denote current batch as $\mathcal{D}$ which is drawn from the union of current training set $\mathcal{D}_t$ and the buffer set $\mathcal{M}$ at task $t$. The instance-wise similarity vector $\mathbf{p}(\cdot)$ for an arbitrary sample $\mathbf{x}_{i} \in \mathcal{D}$, trained model weights $\psi$, and temperature hyperparameter $\kappa$ is defined as follows:

% where 
% \begin{align}
% p_{i, j}&=\frac{\exp \left(\mathbf{z}_{i} \cdot \mathbf{z}_{j} / \kappa\right)}{\sum_{k \neq i}^{2N} \exp \left(\mathbf{z}_{i} \cdot \mathbf{z}_{k} / \kappa\right)}, \\
% \mathbf{z}_{i} &= (g \circ f)_{\psi}(\tilde{\mathbf{x}}_{i}), \qquad
% j \neq i  
% \end{align}
%Note that the instance-wise similarity vector $\mathbf{p}(\cdot)$ represents the feature relation between one view to others with respect to trained model weights $\psi$.
%In the end, Distillation of instance-wise relation from one model to another can be defined as follows:
%\begin{align}
%\label{eqn:IRD}
%    &\mathcal{L}^{\text {IRD }}(\mathcal{B};\psi^{\ast}, \psi, \kappa^{\ast}, \kappa) \nonumber\\
%    &=\sum_{i=1}^{2N}-\mathbf{p}\left(\tilde{\mathbf{x}}_{i} ; \psi^{\ast}, \kappa^{\ast}, \mathcal{B}\right) \cdot \log \mathbf{p}\left(\tilde{\mathbf{x}}_{i} ; \psi, \kappa, \mathcal{B}\right)
%\end{align}
%where ${\psi}$ and ${\kappa}$ denote model weights and temperature hyperparameter, respectively, and the ones with a superscript ${\ast}$ indicate reference model and temperature hyperparameter. 
% The detailed comparison between \cite{fang20} and ours are provided in the supplementary material.

By using fixed model weights snapped at the end of previous task training as the reference model $\psi^{\text{past}}$, IRD distills learned representations to the current training model $\psi$, thereby leading to preserving learned representations. Since contrastive representation learning stems from deep metric learning, IRD achieves knowledge preservation by regulating overall \textit{structure} changes of learned representations. Note that IRD does not regulate exact changes in feature space and does not define relation from encoder outputs like \cite{fang20}. More detailed comparisons between \cite{fang20} and ours are provided in the supplementary material.
% We remark that our instance-wise relation knowledge distillation can be used to preserve learned representations by using fixed model weights snapped at the end of previous task training as reference model ($\psi^\ast$). 
% In the end, by combining asymmetric supervised contrastive loss and IRD, the total loss is defined as follows:
% \begin{align}
% \label{eqn:total-loss}
%     &\mathcal{L} = \mathcal{L}^\text{sup}_\text{asym} + \lambda \mathcal{L}^{\text{IRD}}
% \end{align}
% where $\lambda$ is a hyperparameter to control distillation power.
% Although highly transferable representations suffer less from forgetting, forgetting is inevitable while learning new representations unless regulate the changes in learned ones.
% Note that IRD does not regulate exact changes in feature space. Since contrastive representation learning stems from deep metric learning, IRD achieves knowledge preservation by regulating overall \textit{structure} of learned representation. More details are provided in supplementary material.

% However, simply regulating the changes of learned features of past samples can hinder one's model from learning new representation. 
% Since contrastive representation learning stems from deep metric learning and shows its effectiveness of transferable representations, the structure of representations itself might represent what models learned. Thus the knowledge preservation can be performed by regulating overall structure of learned representations, which IRD actually achieves. 

% \begin{figure}[t]
% \begin{center}
% \centerline{\includegraphics[width=0.85\columnwidth]{figure/ird_asym.png}}
% \caption{The test accuracy after training the last task of Seq-CIFAR-10 on two training schemes: original SupCon and Asymmetric SupCon loss. Both settings use all past task samples on both representation learning and linear classifier training. Note that the red line indicates the upper bound performance. Instance-wise Relation Distillation (IRD) effectively closes the performance gap, which indicates IRD successfully retains learned representation without using past samples as positive pairs.}
% \label{fig:ird_asym}
% \end{center}
% \end{figure}

% We simply verify that IRD can preserve learned representation though we use the main learning objective as asymmetric supervised contrastive loss (Section~\ref{subsection:asymsup}). We consider synthetic scenario that all past samples are available both on representation learning and linear classifier training. Under this setting, we compare two training schemes on Seq-CIFAR-10 (Section~\ref{subsection:exp_setup}): one with original supervised contrastive loss (eq.~\eqref{eqn:supcon}) and the other with asymmetric supervised contrastive loss (eq.~\eqref{eqn:supcon_asym}). As shown in Figure~\ref{fig:ird_asym}, without IRD, i.e., $\lambda=0$, learned representations are not maintained well. With increasing IRD power, however, the performance gap between two learning schemes are closing, which indicates IRD successfully preserves learned representations without using past samples as positive pairs in contrastive objective. 

% Note that the expression and our distillation loss are inspired by \cite{fang20}. 
% The self-supervised distillation loss  \cite{fang20} aims to distill knowledge from teacher models trained on contrastive representation learning scheme to student models which are typically smaller models. 
% Ours are, however, different from \cite{fang20} in that similarity vectors are defined on batch samples and normalized projection; \cite{fang20} use an additional queued samples and normalized encoder outputs to define similarity vectors. 
% The detailed comparison between \cite{fang20} and ours are provided in the supplementary material.


==> arxiv_Contrastive Continual Learning/Method/base.tex <==

\label{section:method}
Here, we propose a rehearsal-based contrastive continual learning scheme, coined \textbf{Co$^2$L} (\textbf{Co}ntrastive \textbf{Co}ntinual \textbf{L}earning). At a high level, Co$^2$L (1) \textit{learns} the representations with an asymmetric form of supervised contrastive loss (Section~\ref{subsection:asymsup}) and (2) \textit{preserves} learned representations using self-supervised distillation (Section~\ref{subsection:IRD}) in a decoupled representation-classifier training scheme. This is done by a mini-batch gradient descent based on the compound loss 
\begin{align}
\label{eqn:total-loss}
    &\mathcal{L} = \underbrace{\mathcal{L}^\text{sup}_\text{asym}}_\text{(1) learning} + 
    \underbrace{\vphantom{\mathcal{L}^\text{sup}_\text{asym}}\lambda\cdot \mathcal{L}^{\text{IRD}}}_{\text{(2) preserving}}.
\end{align}
Here, each batch is composed of two independently augmented views of $N$ samples (thus $2N$ in total), where each sample is drawn from the union of current task samples and buffered samples.

\input{Method/supcon}

\input{Method/IRD}

\input{figures_tex/observation}

\input{Method/wrapup}

==> arxiv_Contrastive Continual Learning/Method/supcon.tex <==
\subsection{Representation Learning with Asymmetric Supervised Contrastive Loss}
\label{subsection:asymsup}

For learning representation continually, we use an asymmetrically modified version of the SupCon objective $\mathcal{L}^{\text{sup}}$. In the modified version, we only use current task samples as anchors; past task samples from the memory buffer will only be used as negative samples (see Figure~\ref{subfig:asymsup}). Formally, if we let $S \subset \{1,\ldots,2N\}$ be the set of indices of current task samples in the batch, the modified supervised contrastive loss is defined as
\begin{align}
    \label{eqn:supcon_asym}
    \mathcal{L}^{\text {sup }}_{\text{asym}} &=\sum_{i \in S}  \frac{-1}{|\mathfrak{p}_i|} \sum_{p \in \mathfrak{p}_i} \log \frac{\exp \left(\mathbf{z}_{i} \cdot \mathbf{z}_{p} / \tau\right)}{\sum_{k \ne i} \exp \left(\mathbf{z}_{i} \cdot \mathbf{z}_{k} / \tau\right)}.
\end{align}
The motivation behind this asymmetric design is to prevent a model from overfitting to a small number of past task samples. It turns out that such a design indeed helps to boost the performance. In Section~\ref{subsection:ablation}, we empirically observe that the asymmetric version $\mathcal{L}^{\text{sup }}_{\text{asym}}$ outperforms the original $\mathcal{L}^{\text{sup}}$ and generates better-spread features of buffered samples.

%We continually learn representation by modifying the existing SupCon objective (eq.~\eqref{eqn:supcon}) to an asymmetric form (eq.~\eqref{eqn:supcon_asym}). 
%Specifically, with the set of indices of batch samples $I$ and a set of indices of current task samples $S \subset I$, the modified asymmetric supervised contrastive loss is defined as follows:
%\begin{align}
%\label{eqn:supcon_asym}
%    \mathcal{L}^{\text {sup }}_{\text{asym}} &=\sum_{i \in S}  \frac{-1}{|\mathfrak{p}_i|} \sum_{p \in \mathfrak{p}_i} \log \frac{\exp \left(\mathbf{z}_{i} \cdot \mathbf{z}_{p} / \tau\right)}{\sum_{k \ne i} \exp \left(\mathbf{z}_{i} \cdot \mathbf{z}_{k} / \tau\right)}
%\end{align}

%The main difference between proposed $\mathcal{L}^{\text {sup }}_{\text{asym}}$ and $\mathcal{L}^{\text {sup }}$ is the samples used as positive anchors/pairs; $\mathcal{L}^{\text {sup }}_{\text{asym}}$ uses only current task samples as positive anchors/pairs. As we will show the empirical effectiveness of $\mathcal{L}^{\text {sup }}_{\text{asym}}$ in Section~\ref{subsection:main-results}, proposed loss helps models to achieve discriminative power among tasks while preventing learned representations from severely drifting by the limited number of past task samples. 
% We will empirically show the effectiveness of proposed asymmetric SupCon loss over the original one in Section~\ref{subsection:asym-supcon}. 



% {\color{blue}Based on our novel observation in Section \ref{subsection:observation}, we choose to} continually learn transferable representation on supervised contrastive learning scheme \cite{khosla20} (SupCon). 
% {\color{blue}Yet, na\"{i}vely optimizing SupCon objective on current batch samples can hurt learned representation: the feature space quickly changes as those limited number of samples play as positive anchors and thus get closer to each other. However, it is not desirable to optimize SupCon objective only on samples associated with current task since discriminative power between different tasks can be achieved when those play as negative pairs.} 

% Although our asymmetric supervised contrastive loss can help our model continually learning new knowledge while achieving discriminative power among tasks, one may doubt whether such loss can sufficiently preserve learned representation since it leaves out past task samples from being used as positive pairs. To cope with this, in the later Section~\ref{subsection:IRD}, we will describe how our method \textit{preserve} learned representation. 

==> arxiv_Contrastive Continual Learning/Method/wrapup.tex <==
\subsection{Algorithm Details}
\label{subsection:Co$^2$L}
\input{algorithm/whole}
Here, we give a complete picture of the overall training procedure and give additional details. The full algorithm is provided in Algorithm \ref{alg:whole}. 

\vspace{0.2em}
\noindent\textbf{Data preparation.} 
As the initial or new task arrives, the dataset is built as a union of current task samples and buffered samples, without any oversampling \cite{Chawla02, han05}. The mini-batch is drawn from this dataset, where each sample is independently drawn with equal probability. To enjoy the benefits of contrastive representation learning, each sample is augmented into two views following \cite{Chen19}. The detailed augmentation scheme for contrastive learning is provided in the supplementary material.

\vspace{0.2em}
\noindent\textbf{Learning new representation.} The augmented samples are forwarded to the encoder $f_{\vartheta}$ and projection map $g_{\phi}$ sequentially. The projection map outputs are used to compute asymmetric supervised contrastive loss (eq.~\ref{eqn:supcon_asym}).

% \input{algorithm/buffer}

\vspace{0.2em}
\noindent\textbf{Preserving learned representation.}
When a new task arrives (\ie, $t > 1$), we compute instance-wise relation drifts between reference model and the training model with IRD loss (eq.~\ref{eqn:IRD}). To this end, we settle the reference model as the trained model at the end of the training of $(t-1)$-th task. Note that while optimizing total loss (eq.~\ref{eqn:total-loss}), the reference model is not updated.

\vspace{0.2em}
\noindent\textbf{Buffer management.}
At the end of training each task, a small portion of training samples is pushed into a replay buffer. Due to its buffer size constraint, a small subset of samples from each class is pulled out of the replay buffer at the same ratio. The sample to be pushed or pulled is uniformly randomly selected for all procedures.



==> arxiv_Contrastive Continual Learning/Observation/observation.tex <==
\subsection{Main Results}\label{subsection:observation}

% In this sense, prior studies often pose more importance on one of those concerns than the other, \eg, learn new knowledge which does not contradict to previously acquired one. 

\noindent\textbf{Validation on our key hypothesis.}
%Contrastively learned representations less suffer from forgetting.}
Before we provide results of Co$^2$L in comparison with other methods, we first validate our running premise for method design: \textit{Contrastive learning learns more useful representation for the future task than the joint classifier-representation supervised learning.} This premise, however, is not easy to verify under the standard continual learning setup. Indeed, the quality of a representation is typically defined as the joint predictive performance with the best possible (linear) downstream classifier (see, \eg, \cite{arora19}, and references therein), but optimal classifiers are only rarely learned under continual setups.

To circumvent this obstacle, we consider the following synthetic, yet insightful scenario: After training representations under the standard continual setup, we freeze the representations and freshly train the downstream classifier, using training data from \textit{all tasks}. Here, the classifier trained on all observed samples so far will perform learned tasks well unless frozen representations suffer from forgetting.

% compare the quality of contrastively learned representations (hereinafter referred to as \textit{contrastive}) with the representation learned by a standard joint classifier-representation training (referred to as \textit{joint}), under a 


%The major concern on continual learning problem is how to acquire new knowledge while preventing catastrophic forgetting. However, it gets less attention which type of knowledge to be learned across tasks. We remark that the continual learning settings where the access to samples is limited do hold not only on past samples but also on future samples. Namely, if models try to learn representation useful for the unseen tasks, such representation would be more sustainable, leading to less forgetting. Hence, the transferable representation is worth being learned and also itself would suffer less from forgetting. 
%
%Such strategies innately assume that it is inevitable to sacrifice one for the other. 
%
% Under the settings where the access to past samples is restricted, prior studies in continual learning mainly focus on regulate knowledge acquisition to protect learned knowledge which is more vulnerable to forgetting. 
%
%

% We empirically demonstrate the benefits of transferable knowledge mentioned above as follows. We basically compare two learning schemes. We denote the encoder-classifier joint training scheme by \textit{joint} and the encoder contrastive training scheme by \textit{contrastive}. One can expect that the reprsentation from \textit{contrastive} is more transferable than the one from \textit{joint}. Following the conventional class incremental learning settings, we sequentially train ResNet-18 as an encoder of each scheme on Seq-CIFAR-10 which consists of 5 disjoint sets of 2 class samples of CIFAR-10. After each task ends, a new randomly initialized linear classifier is trained and tested on top of trained encoder under two settings: (1) use samples observed so far and (2) use all samples including ones from unseen tasks, each of which corresponds left and right pair of heatmaps in Figure \ref{fig:observation}, respectively. Note that we don't re-intialize weight parameters after training each task.

As shown in the left pair of heatmaps in Figure \ref{fig:observation}, the average test accuracy on the previous tasks is surprisingly higher in \textit{contrastive} than in \textit{joint} (for off-diagonal parts, 21.79\% vs. 66.46\%). In other words, without any specific method to account for continual setup, contrastive method learns representations that suffer less from forgetting than jointly trained ones. 

In the right pair of heatmaps in Figure~\ref{fig:observation}, we report test accuracies of the classifiers that are trained with \textit{all samples}, including the samples from unseen tasks.
Interestingly, we observe that the average task accuracy on the unseen task is also notably higher in contrastively trained representations (rightmost heatmap) than jointly trained ones (second to right); for lower triangle parts, 32.77\% vs. 62.76\%. This implies that contrastive learning methods learn more highly transferable representations to future tasks, which might be the source of its robustness against forgetting.
%Meanwhile, we also train classifiers with all samples including ones from unseen tasks to validate whether contrastively learned representation is useful for the unseen tasks.
%Interestingly, we observe that the average test accuracy on the unseen task is also higher in \textit{contrastive} in the right pair of heatmaps in Figure \ref{fig:observation} (for lower triangular part, 32.77\% vs. 62.76\%). This implies that highly transferable representations contain more useful information to be leveraged in the future, which might be the source of its tolerance against forgetting.


% It gets, however, less attention whether learned knowledge itself is useful enough to regulate future learning procedure. 
% Namely, one can expect that a continually trained model gets susceptible to learn new knowledge when it already has learned transferable knowledge, whereby would lead this model to suffer less from forgetting. 
%, whereby leads to stability - plasticity dilemma.
% Does knowledge acquisition inevitably prone models to forget learned representation? 


% We thus choose to leverage contrastive representation learning schemes to acquire highly transferable representation upon coventional continual learning settings. We first train ResNet18 with the supervised contrastive loss for 5 tasks, each of which consists of CIFAR-10 samples of 2 classes, in a sequential manner. After training each task, we train a linear classifier on training samples observed so far on top of the encoder of trained models. We conduct this procedure  
% We conduct exactly the same procedure with cross entropy loss as the objective. 

% As shown in Figure \ref{fig:observation}, one can observe that the performance with contrastive learning scheme is consistently higher than the one with typical supervised learning scheme. This indicates that contrastively learned knowledge less suffers forgetting even without replaying samples during representation learning. 

% \citet{Chen19} pointed out that it is crucial to incentivize our model to preserve learned knowledge since 
% As \citet{Chen19} pointed out, however, it is substantial to incentivize our model to preserve learned representation since 
% it is not convincing that such representation learning schemes on the continual learning setup directly incentivize our model to preserve learned representation, which is crucial . Hence, in the following sections, we'll propose explicitly designed training scheme for contrastive continual learning.



% prone to maintain learned representations after sequential training since they do not explicitly incentivise to preserve representation that is not useful to perform current task but learned previously. 












%In contrast, if any learning scheme is able to acquire representation that is generalizable to perform given any task, the main concern moves toward maintaining its representation since naive training schemes hardly incentivise the model to preserve this knowledge.  

% Such dilemma easily occurs when one model is trained on canonical joint training scheme, i.e., optimizing cross entropy loss on the encoder and classifier. This is because such training scheme learns representation that efficiently demonstrates 


==> arxiv_Contrastive Continual Learning/abstract.tex <==
%
% Prior studies make efforts to keep past signals to mitigate forgetting with their own strategies, e.g., exemplar rehearsal, weight regularization.
% {\color{blue} JH: what do you want to say with this sentence? Are you trying to say that `continual learning is an important problem; many people worked on this problem.' Or, are you trying to say `Prior strategies focus on keeping past signals, while ours do not'? In the abstract (and in any writing), it is desirable to keep only the sentences that are written with intentions, and remove any gap-filler sentences that plays no clear role.}
%
% Yet, existing strategies generally follow joint learning scheme, i.e., training representations and classifiers jointly, and only a few studies consider learning representation which is robust itself to forgetting.
% {\color{blue} JH: Why does ``joint learning'' suck? Why is ``learning representation'' cool? Why should we even consider learning representation separately?}
%
% In this paper, we propose a continual representation learning scheme that enjoys benefits of contrastive representation learning scheme.
% {\color{blue}JH: I see. So the goal is to come up with a ``representation'' not the whole classifier. The keyword ``contrastive,'' though, feels like it came out of nowhere.}
%
% We first observe representation contrastively learned has more potential to retain its discriminative power than jointly trained ones.
% {\color{blue}This sentence provides a (partial) answer to the question I raised. But perhaps we should make clear what setup we consider, e.g., what we have an access to.}
%
% Based on our novel observation, we propose contrastive continual learning scheme leveraging self-supervised distillation to preserve instance-wise relation through multiple tasks.
%
%
% DER
% Continual Learning has inspired a plethora of approaches and evaluation settings;
% however, the majority of them overlooks the properties of a practical scenario,
% where the data stream cannot be shaped as a sequence of tasks and offline training
% is not viable. We work towards General Continual Learning (GCL), where task
% boundaries blur and the domain and class distributions shift either gradually or
% suddenly. We address it through mixing rehearsal with knowledge distillation
% and regularization; our simple baseline, Dark Experience Replay, matches the
% network’s logits sampled throughout the optimization trajectory, thus promoting
% consistency with its past. By conducting an extensive analysis on both standard
% benchmarks and a novel GCL evaluation setting (MNIST-360), we show that such
% a seemingly simple baseline outperforms consolidated approaches and leverages
% limited resources. We further explore the generalization capabilities of our objective, showing its regularization being beneficial beyond mere performance.
% Code is available at https://github.com/aimagelab/mammoth.
%
%
%
% The human-like ability to continually learn new knowledge is challenging in deep learning based classification models due to catastrophic forgetting. 
%
% The fundamental challenges in the continual learning problem stem from limited accessibility to observed/unknown samples at arbitrary training phase. 
%
% Hence, learning task-agnostic and universally transferable knowledge across tasks can be substantial to train models continually. 
%
% In that sense, one can leverage recent progress in representation learning schemes to acquire such knowledge. 
%
% We thus first apply contrastive representation learning schemes that often even show better performance than one with supervised training under traditional continual learning settings. 
%
% We observe that contrastively learned representation is more robust to forgetting even without any tailored design for continual learning. 
%
% Based on this observation, we propose a continual representation learning scheme that enjoys the benefits of contrastively learned representation. 
%
% By additionally accessing only a small portion of observed past samples, we explicitly maintain instance-wise relations involved in learned representation in a self-supervised distillation manner. 
%
% We conduct extensive experiments and set new state-of-the-art performance on continual learning benchmarks CIFAR-10, CIFAR-100, and Tiny-ImageNet.

% Catastrophic forgetting has been a long-standing problem in settings where access to past or future samples is limited. But, is forgetting always inevitable in these settings?
% Recent breakthroughs in un/self-supervised representation learning demonstrate that this type of learning scheme gives a better transferable knowledge than the one jointly trained on task-specific supervision.
Recent breakthroughs in self-supervised learning show that such algorithms learn visual representations that can be transferred better to unseen tasks than joint-training methods relying on task-specific supervision.
In this paper, we found that the similar holds in the \textit{continual learning} context: contrastively learned representations are more robust against the catastrophic forgetting than jointly trained representations. 
Based on this novel observation, we propose a rehearsal-based continual learning algorithm that focuses on continually learning and maintaining transferable representations. 
More specifically, the proposed scheme (1) \textit{learns} representations using the contrastive learning objective, and (2) \textit{preserves} learned representations using a self-supervised distillation step.
We conduct extensive experimental validations under popular benchmark image classification datasets, where our method sets the new state-of-the-art performance.


==> arxiv_Contrastive Continual Learning/algorithm/buffer.tex <==

\begin{algorithm}[H]
\caption{Buffer manage algorithm}
\label{alg:buffer}
\begin{algorithmic}[1]

\STATE \textbf{Input}: Buffer size $M$, buffer $\mathcal{M}:=\{(x_i, y_i)\}^M_{i=1}$, a set of current $t$ task samples $\mathcal{D}_t$, a set of disjoint class sets so far $\{\mathcal{C}_k\}^t_{k=1}$.

\STATE TBD
\end{algorithmic}

\end{algorithm}


==> arxiv_Contrastive Continual Learning/algorithm/whole.tex <==

\begin{algorithm}[t]
\caption{Co$^2$L: Contrastive Continual Learning}
\label{alg:whole}
\begin{algorithmic}[1]
% \begin{multicols}{2}

\STATE \textbf{Input}: 
Encoder parameters $\vartheta$, 
projector parameters $\phi$, 
number of tasks $T$, 
family of augmentations $\mathcal{H}$,
a set of training sets $\{\{(x^t_i, y^t_i)\}\}^T_{t=1}$, 
a set of disjoint class sets $\{\mathcal{C}_t\}^T_{t=1}$, 
learning rate $\eta$, 
number of epochs of $t$-th task $E_t$, 
% parameter update momentum $m$, 
distillation temperatures $\kappa,\kappa^{\ast}$, 
distillation power $\lambda$.

\STATE Initialize network $(g \circ f)_{\psi} (\cdot)$ where $\psi = (\vartheta,\phi)$.
\FOR{$t = 1, \cdots, T$}

\STATE Construct dataset $\mathcal{D}$ by $\mathcal{D} \gets \{(x^t_i, y^t_i)\} \cup \mathcal{M}$\\


% \IF {$t > 1$}
% \STATE Prepare momentum parameter updates \\
% \STATE $\psi^t_0 \gets \psi^{t-1}_E$
% \STATE $\psi^{t-1}_0 \gets \psi^{t}_0$
% \ENDIF

\FOR{$e = 1, \cdots, E_t$}

\STATE Draw a mini-batch $\{(x_i, y_i)\}_{i=1}^{N}$ from $\mathcal{D}$\\

% \COMMENT{Construct augmented mini-batch set}
\FORALL{$k \in \{1, \cdots ,N\}$}
\STATE Draw two augmentations $h\sim\mathcal{H}, h'\sim\mathcal{H}$ \\
\STATE Initialize 
% augmented sample set $\mathcal{R} \gets \emptyset$, \\ and 
anchor indices sets $S \gets \emptyset, I \gets \emptyset$
% $\mathcal{S} \gets \emptyset$ \\
\STATE $\tilde{x}_{2k-1} = h(x_k)$\\
\STATE $\tilde{x}_{2k} = h'(x_k)$\\
% \STATE $\mathcal{R} \gets \mathcal{R} \cup \{(\tilde{x}_{2k-1}, y_k), (\tilde{x}_{2k}, y_k)\}$\\
\STATE $I \gets I \cup \{2k-1, 2k\}$
\IF {$y_k \in C_t$}
\STATE $S \gets S \cup \{2k-1, 2k\}$
\ENDIF
\ENDFOR

\STATE Compute $\mathcal{L}$ by $\mathcal{L} \gets \mathcal{L}^\text{sup}_\text{asym}(I, S; \psi^{t}_{e-1})$ (eq.~\ref{eqn:supcon_asym})\\
\IF {$t > 1$}
\STATE Update $\mathcal{L}$ by \\ $\mathcal{L} \gets \mathcal{L} + \lambda \cdot \mathcal{L}^\text{IRD}(\psi^{t-1}_{E_{t-1}}, \psi^{t}_{e-1}, \kappa^{\ast}, \kappa)$ (eq.~\ref{eqn:IRD})
\ENDIF

\STATE Update 
$\psi^t_{e-1}$
% $(g \circ f)_{\psi^t_{e-1}} (\cdot)$ 
by $\psi^t_{e} \gets \psi^t_{e-1} - \eta \nabla_{\psi^t_{e-1}} \mathcal{L}$ \\
% \STATE $\psi^{t-1}_e \gets m\psi^{t-1}_{e-1} + (1-m)\psi^t_e $\\
\ENDFOR

\STATE Manage buffer $\mathcal{M}$ for the number of each class samples to be same by uniform sampling.
% with $\{(x^t_i, y^t_i)\}$ (Algorithm \ref{alg:buffer})
\ENDFOR
% \end{multicols}
\end{algorithmic}
\end{algorithm}
\vspace{-0.5em}

==> arxiv_Contrastive Continual Learning/conclusion.tex <==
\label{section:conclusion}
We propose a contrastive continual learning scheme for learning representations under continual learning scenarios. The proposed asymmetric form of contrastive learning loss and the instance-wise relation distillation help model learn and preserve new and past representations and show a better performance over jointly trained baselines on various learning setups. We hope that our work will serve as a good reference to how representation learning for continual learning should be designed.


==> arxiv_Contrastive Continual Learning/figures_tex/asym_tiled.tex <==
\begin{figure}
\begin{center}
\centerline{\includegraphics[width=0.8\columnwidth]{figure/asym_tiled.png}}
\caption{Top: $t$-SNE visualization of features from buffered (colored) and entire (gray) training samples of Seq-CIFAR-10. Bottom: Same as Top, but non-buffered samples are in opaque color instead of gray for a clear illustration of clusters. Left: Buffered samples' features trained with original SupCon are close to the same class samples but distant from different classes. Right: Buffered samples' features trained on asymmetric SupCon are well-spread; buffered samples better represent the entire class sample population.
}
\label{fig:ablation_asym_sup}
\end{center}
\vspace{-3em}
\end{figure}


==> arxiv_Contrastive Continual Learning/figures_tex/ird_asym.tex <==
\begin{figure}
\begin{center}
\centerline{\includegraphics[width=0.85\columnwidth]{figure/ird_asym.png}}
\caption{ Performance comparison of original and asymmetric SupCon losses on Seq-CIFAR-10 under the ideal class-IL scenario. Both settings use \text{all} past task samples. Instance-wise Relation Distillation (IRD) effectively closes the performance gap, which indicates IRD successfully retains learned representations without using past samples as positive pairs.}
\label{fig:ird_asym}
\end{center}
\vspace{-2em}
\end{figure}

==> arxiv_Contrastive Continual Learning/figures_tex/main_fig.tex <==
\begin{figure*}
\vspace{-1em}
\begin{center}
\centerline{\includegraphics[width=0.9\textwidth]{figure/cocoa_all.png}}
\caption{An overview of the Co$^2$L framework. Mini-batch samples from the current task and the memory buffer are augmented and passed through current and past (stored at the end of the previous task) representations. Co$^2$L minimizes the weighted sum of two losses: (1) Asymmetric SupCon loss contrasts anchor samples from the current task against the samples from other classes (Section~\ref{subsection:asymsup}). (2) IRD loss measures the drift of the instance-wise similarities given by the current model from the one given by the previous model (Section~\ref{subsection:IRD}).}
\label{fig:mainfig}
\end{center}
\vspace{-2.5em}
\end{figure*}

==> arxiv_Contrastive Continual Learning/figures_tex/observation.tex <==
\begin{figure*}
\begin{center}
\centerline{\includegraphics[width=\textwidth]{figure/observation2.png}}
\caption{Observation on two learning schemes, representation-classifier joint training and contrastive representation learning on Seq-CIFAR-10 without any design used for the continual learning settings. As new task arrives, each model is trained only with current task samples with model weights without re-initialization. After each task training ends, a new linear classifier is trained on the fixed current representation with samples observed so far (denoted by ``seen objects'') or all samples including ones from future tasks (denoted by ``all objects''). The pair of left figures shows contrastively trained representations suffer less from forgetting than the joint trained ones. The right pair shows contrastively learned representation is much more useful to perform unseen objects classification tasks.}
\label{fig:observation}
\end{center}
\vspace{-2em}
\end{figure*}

==> arxiv_Contrastive Continual Learning/figures_tex/submethods.tex <==
% \begin{figure*}
% \begin{center}
% \centerline{\includegraphics[width=0.9\textwidth]{figure/IRD4.png}}
% \caption{ Illustration of Instance-wise Relation Distillation (IRD). Given augmented mini-batch samples, the instance-wise relation is defined on the normalized projected feature vectors. The relation vectors, \ie, dot products ($\odot$) of feature vectors, are computed from the learnable ($\psi^t_{e-1}$) and reference model ($\psi^{t-1}_{E}$), respectively. For $E$ epoch training, such temperature scaled relation is distilled from the reference model to the learnable model. Note that the reference model is snapped at the end of $(t-1)$\textit{-th} task training, and we only update the learnable model's weights using stop-gradient (denoted by $\mathtt{sg}$).}
% \label{fig:IRD}
% \end{center}
% \vspace{-2em}
% \end{figure*}


\begin{figure*}[t]
\vspace{-1em}
\centering
\subfigure[Asymmetric SupCon Loss]{
\centering
\includegraphics[height=1.8in]{figure/ASYM6.png}
\label{subfig:asymsup}
}
\subfigure[Instance-wise Relation Distillation Loss]{
\centering
\includegraphics[height=1.8in]{figure/IRD6.png}
\label{subfig:ird}
}
\caption{
Illustration of Asymmetric Supervised Constrastive Loss and Instance-wise Relation Distillation (IRD). (a) Given augmented mini-batch samples, asymmetric SupCon considers samples from the same class of the current task as positives. In other words, the pulling effects between anchors only exist between current task samples. (b) Given augmented mini-batch samples, the instance-wise relation is defined on the normalized projected feature vectors. The relation vectors, \ie, dot products ($\odot$) of feature vectors, are computed from the learnable ($\psi^t_{e-1}$) and reference model ($\psi^{t-1}_{E}$), respectively. For $E$ epoch training, such temperature scaled relation is distilled from the reference model to the learnable model. Note that the reference model is snapped at the end of $(t-1)$\textit{-th} task training, and we only update the learnable model's weights using stop-gradient (denoted by $\mathtt{sg}$).}
\label{fig:submethods}
\vspace{-0.5em}
\end{figure*}

==> arxiv_Contrastive Continual Learning/intro.tex <==
\input{figures_tex/main_fig}


Modern deep learning algorithms show impressive performances on the task at hand, but it is well known that they often struggle to retain their knowledge on previously learned tasks after being trained on a new one \cite{mccloskey89}. To mitigate such ``catastrophic forgetting,'' prior works in the continual learning literature focus on \textit{preserving} the previously learned knowledge using various types of information about the past task. Replay-based approaches store a small portion of past samples and rehearse the samples along with present task samples \cite{robins95,lopezpaz17,riemer19,buzzega20}. Regularization-based approaches force the current model to be sufficiently close to the past model---which may be informative about the past task---in the parameter/functional space distance \cite{kirkpatrick17,chaudhry18,serra18}. Expansion-based approaches allocate a unit (\eg, network node, sub-network) for each task and keep the unit untouched during the training for other tasks \cite{rusu16,mallya18}.

%In modern times, deep learning has become excellent at performing a given task, but deep neural networks still suffer forgetting what they learned while learning new knowledge, so called catastrophic forgetting. To mitigate such serious phenomenon, prior work in continual learning mostly focuses on preventing forgetting under settings where the access to past samples is limited. Replay-based approaches rehearse a small portion of past samples to overcome such limited accessibility in data space, and regularization-based approaches regulate the changes in parameter or functional space to keep learned knowledge. Recent studies further develop such strategies under more realistic settings where the task boundary or identifier is not available. 

In this paper, instead of asking how to isolate previous knowledge from new knowledge, we draw attention to the following fundamental question:
\vspace{0.1in}
\begin{quotation}\em
What type of knowledge is likely to be useful for future tasks (and thus not get forgotten), and how can we learn and preserve such knowledge?
\end{quotation}
\vspace{-0.1in}
To demonstrate its significance, consider the simple scenario that the task at hand is to classify the given image as an apple or a banana. An easy way to solve this problem is to extract and use the color feature of the image; red means apple, and yellow means banana. The color, however, will no longer be useful if our future task is to classify another set of images as apples or strawberries; color may not be used anymore and eventually get forgotten. On the other hand, if the model had learned more complicated features, \eg, shape/polish/texture, the features may be re-used for future tasks and remain unforgotten. This line of thoughts suggests that forgetting does not only come from the limited access to the past experience, but also from the innately restricted access to future events; to suffer less from forgetting, learning more \textit{transferable representations} in the first hand may be as important as carefully preserving the knowledge gained in the past.

%While most of studies consider the gist of continual learning problem as isolating learned knowledge from new knowledge, in this work, we cast following questions instead: which type of knowledge should be learned and how to learn such knowledge? To demonstrate, let us suppose our model tries to classify apple from banana. This easy classification problem can be solved by using only color information in visual inputs. Such information, however, will be no longer useful to classify apple from strawberry, which would be the future tasks. However the minimum information is enough to perform current task, \eg, colors for apple and banana, humans make decision utilizing the more complex and rich information, \eg, shape, polish and pattern of objects. This simple line of thoughts implies that forgetting not only comes from the limited accessibility to past experience but also comes from the unexpected and innately restricted accessibility to future events. Hence, the knowledge useful for future tasks might be suffer less from forgetting so that it is desired to train our model to acquire such useful knowledge. 

To learn more transferable representations for continual learning, we draw inspirations from a recent advance in self-supervised learning, in particular, \textit{contrastive learning} \cite{hadsell06,chen20}. Contrastive methods learn representations using the inductive bias that the prediction should be invariant to certain input transformations instead of relying on task-specific supervisions. 
Despite their simplicity, such methods are known to be surprisingly effective;
for ImageNet classification \cite{ILSVRC15}, contrastively trained representations closely achieve the fully-supervised performance even without labels \cite{chen20} and outperform joint-trained counterparts in the supervised case \cite{khosla20}.
More importantly, while the methods are originally proposed for better in-domain\footnote{The term `in-domain' is used here for the setup where data distributions for representation learning and linear classifier training are the same.} 
performance, recent works also show that such methods provide significant performance gains on unseen domains \cite{chen20,he20}.
%Although contrastive methods learn representations without task-specific supervision, recent breakthroughs \cite{chen20, khosla20} in this literature achieve competitive or even higher performance on image classification tasks on popular benchmarks, \eg, the ImageNet \cite{ILSVRC15}, upon their contrastively trained representations than the ones with jointly trained under supervised cross-entropy training.
% , \eg, the ImageNet classification task performance of linear classifiers trained upon SimCLR pretrained representations achieves 76.5\% top-1 accuracy. 
% For instance, in image classification tasks, contrastive learning schemes on the ImageNet dataset show a top-1 accuracy of 70.2\% and 78.7\% of linear classifiers on representations trained on the unsupervised \cite{chen20} and supervised \cite{khosla20}, which is competitive compared to 78.0\% of standard cross-entropy training.
%Also, while contrastive methods are originally proposed for better in-domain\footnote{The term `in-domain' is used here for the setup where the datasets for representation learning and linear classifier training are the same.} performance, recent works show that such methods provide significant performance gains on unseen domains \cite{chen20,he20}. 
Under a continual scenario, we make a similar observation: 
\textit{contrastively learned representations suffer less from forgetting than the jointly trained ones} (see Section~\ref{subsection:observation} for details).
% As we will  show in Section~\ref{subsection:observation}, we observe that the similar holds:
% \textit{contrastively learned representations suffer less from forgetting than the jointly trained ones}.

Unfortunately, applying this idea to continual settings is not straightforward due to at least two reasons: First, having access to informative negative samples is known to be crucial for the success of contrastive learning \cite{robinson21}, while the instantaneous demographics of negatives samples are severely restricted under standard continual setups; in class-incremental learning, for instance, it is common to assume that the learner can access samples from only a small number of classes at each time step. 
Second, the question of how to preserve the learned \textit{representations} not as a part of a jointly trained representation-classifier pair has not been fully answered. Indeed, recent works on representation learning for continual setups aim to learn representations accelerating future learning under a similar decoupled learning setup but lack an explicit design to preserve representations. 
% {\color{red}... briefly describe the limitations of existing works on representation learning for continual setups.} 



%In this sense, recent progress in un/self-supervised representation learning needs to be considered. Such algorithms are known to learn highly transferable knowledge and often outperform the one trained on joint training schemes relying on task-specific supervision. One can imagine continually trained representations on such schemes will be highly transferable so that it suffer less from forgetting. Hence, the type of representation that neural network learns is an important subject on continual learning settings. Even though there have been some studies of representations in the continual learning problem, most of them focus on designing classifier training schemes to leverage learned representations, the consequential characteristics of representations trained on continual learning algorithm, or just a few of them mainly consider representation learning schemes by leveraging meta learning methodology. 

% Meanwhile, the motivation to leverage un/self-supervised representation learning to solve problems of other research fields has emerged in recent years. 
%\vspace{0.5em}
\noindent\textbf{Contribution.} To address these challenges, we propose a new rehearsal-based continual learning algorithm, coined \textbf{Co$^2$L} (\textbf{Co}ntrastive \textbf{Co}ntinual \textbf{L}earning).
Unlike previous continual (representation) learning methods, we aim to \textit{learn} and \textit{preserve} representations continually in a decoupled representation-classifier scheme. The overview of Co$^2$L is illustrated in Figure~\ref{fig:mainfig}.

Our contribution under this setup is twofold:
% Unlike previous rehearsal-based methods, Co$^2$L utilizes the replay buffer in two different ways:
\begin{enumerate}[leftmargin=*,topsep=0pt,itemsep=-0.5ex,partopsep=1ex,parsep=1ex]
\item \textit{Contrastive learning:} 
We design an asymmetric version of supervised contrastive loss for learning representations under continual learning setup (Section~\ref{subsection:asymsup}) and empirically show its benefits on improving the representation quality. 
% {\color{red}Cite the figure in this paragraph.}
% We first provide novel observation that constrastively learned representations suffer less from forgetting than jointly trained one. Based on this observation, we design modified form of supervised contrastive loss for learning representation continually and empirically show improvement on representation quality.
% {\color{magenta}We enjoy the benefits of contrastive learning framework in the continual learning context based on our novel observation (Section~\ref{subsection:observation}) especially in supervised contrastive loss. We empirically show improvement on representation quality with the modified form of supervised contrastive loss (Section~\ref{subsection:asymsup}).}
% Samples from the previous tasks are used as negatives samples for {\color{blue}both separating new knowledge from past one and preventing severe drifts in learned representation through contrastive learning.} 
%To do this, we propose a novel learning objective designed to handle the innate class imbalance of continual learning setups.
\item \textit{Preserving representations:} 
We propose a novel preservation mechanism for contrastively learned representations, which works by self-distillation of instance-wise relations (Section~\ref{subsection:IRD}); to the best of our knowledge, this is a first method explicitly designed to preserve representations without a jointly trained classifier. 
% {\color{red}Cite the figure in this paragraph.}
%We propose to preserve the contrastively learned representation by novel self-distillation of instance-wise relation (Section~\ref{subsection:IRD}). To the best of our knowledge, ours is the first work that designs explicit representation preservation without classifier joint training.
% Our distillation works without task-specific prior or classifier  does not rely on classifier joint training scheme.
% Co$^2$L preserves the contrastively learned representation by novel self-distillation procedure of instance-wise relations; {\color{blue}samples from the previous tasks plays an essential role in boosting the performance of this distillation procedure.} % We may want to be more specific and argue that the samples "enable a better estimation of some true underlying structure," but we would need evidence for it.
\end{enumerate}
We validate Co$^2$L under various experimental scenarios encompassing task-incremental learning, domain-incremental learning, and class-incremental learning. Co$^2$L consistently outperforms all baselines on various datasets, scenarios, and memory setups.
% For instance, we achieve test accuracy of 74.26\% in class-incremental scenario and 95.90\% in task-incremental scenario on CIFAR-10 with buffer size 500, which is 1.56\% and 2.02\% above the previous state-of-the-art performance of joint training scheme.
With careful ablation studies, we also show that both components we propose (asymmetric supervised contrastive loss, instance-wise relation distillation) are essential for performance.
%We also ablate Co$^2$L to verify two key components, asymmetric supervised contrastive loss and instance-wise relation distillation. 
In the ablation of distillation, we empirically show that distillation preserves learned representations and efficiently uses buffered samples, which might be the main source of consistent gains over all comparisons: distillation provides 22.40\% and 10.59\% relative improvements with/without buffered samples respectively on the Seq-CIFAR-10 dataset. 
% In the ablation of instance-wise relation distillation, we empirically show our distillation loss plays as a key role to preserve learned representations by removing distillation loss with various memory setups. Without buffered samples, distillation provides 5.64\% performance gains and 12.00\% with buffered samples on Seq-CIFAR-10 dataset. This implies that our distillation not only preserves learned representations but also efficiently uses buffered samples, which might be the main source of consistent gain over all comparisons. 
In the ablation of asymmetric supervised contrastive loss, we quantitatively verify that the asymmetric version consistently provides performance gains over the original one on all setups, \eg, 8.15\% relative improvement on the Seq-CIFAR-10 with buffer size 500. We also provide qualitative implication on this performance gain by visualizing learned representations, which shows our asymmetric version prevents severe drifts of learned features.
% In the ablation of asymmetric supervised contrastive loss, we provide both quantitative and qualitative studies to verify asymmetric form successfully provides discriminative power between tasks and prevents severe drifts in learned representations. By simply replacing the original supervised contrastive loss with our asymmetric version, we quantitatively verify ours consistently provides performance gains over all experiment setups, \eg, 5.6\% gains on Seq-CIFAR-10 with buffer size 500. Our qualitative comparison by visualizing representations on Seq-CIFAR-10 samples also shows asymmetric version encourages features of buffered samples to retain its original region in representation space.
% We also visualize representations trained on 
% We also validate the effectiveness of asymmetric version of supervised contrastive loss and instance-wise relation distillation in our ablation studies. 
% Compared to the original supervised contrastive loss, our asymmetric version consistently provides performance gains over all experiment setups, \eg, 5.6\% gains on Seq-CIFAR-10 with buffer size 500. 
% In the ablation of instance-wise relation distillation loss, our distillation provides 5.64\% performance gains without buffered samples and 12.00\% with buffered samples on Seq-CIFAR-10. 
% For the experiments on the more longer sequence of tasks and the domain-incremental scenario we also achieve state-of-the-art performance: Tiny-ImageNet20.12\%(+0.74\%) and 98.65\%(+1.08\%), respectively. 
% {\color{red}Write down what scenarios we consider, and show off the performance; SOTA?}


%\textbf{Contribution.} To mitigate catastrophic forgetting, we propose rehearsal-based continual learning algorithm that focuses on continual learning and maintaining a transferable representation. Our goal is improving continual learning performance on various scenarios with providing novel perspectives on continual representation learning. Specifically, we basically learn highly transferable representation sequentially by following contrastive representation learning schemes in a modified form to effectively learn new representation. Simultaneously, we preserve learned representation by self-distilling the instance-wise relation from reference models. From those learning and preserving steps, it can automatically learn new transferable knowledge while preventing catastrphic forgetting. We validate our algorithm to various learning scenarios and obtain significant improvements over existing continual learning algorithms. Our contributions are as follows

%\begin{itemize}
%    \item We provide novel observation that highly transferable representation suffer less from forgetting. \item Building on this observation, we propose rehearse-based continual learning algorithm that learns and maintain transferable representation. To this end, we propose (1) modified contrastive learning objective to effectively learn new representation and (2) a novel self-distillation loss to preserve instance-wise relation in the feature spaces to prevent forgetting.
%    \item The proposed algorithm achieves significant improvements over existing continual learning algorithms. 
%\end{itemize}

\iffalse
\vspace{0.3em}
\noindent\textbf{Organization.} In Section~\ref{section:related-work}, we discuss related works on continual representation learning and contrastive learning. In Section~\ref{section:background}, we formally describe the considered continual learning setup and give preliminaries on contrastive learning. In Section~\ref{section:method}, we introduce the proposed Co$^2$L. 
In Section~\ref{subsection:exp_setup}, we introduce continual learning setups we consider. 
In Section~\ref{subsection:observation}, we provide a motivational observation that our proposed method mainly concerns, and give experimental results of Co$^2$L under various setups and verify its effectiveness of each component in Section~\ref{subsection:ablation}.
\fi
%The core motivation behind proposed method Co$^2$L is demonstrated in Section~\ref{subsection:observation};
% In Section~\ref{subsection:observation}, we perform a sanity check on the benefit of contrastive learning for continual setup; 
%we show that contrastive methods learn the representations that transfer better to both past and future, than supervised joint-training methods. 
%In the rese of Section~\ref{section:experiment}, we empirically validate its effectiveness in various settings.
% We introduce the proposed Co$^2$L in Section~\ref{section:method}, and empirically validate its effectiveness in Section~\ref{section:experiment}.



%\textbf{Organization}. The rest of the paper is organized as follows. In Section \ref{section:background}, we provide preliminaries on continual learning problems and contrastive representation learning. In Section \ref{section:observation}, we provide our motivational observation and in Section \ref{section:method}, method for contrastive continual learning by components. \ref{section:experiment} shows our experimental results under various settings, and Section \ref{section:conclusion} states the conclusion.

==> arxiv_Contrastive Continual Learning/related_work.tex <==
\label{section:related-work}
\noindent\textbf{Rehearsal-based continual learning.}
Continual learning methods have been developed in three major streams: using a fixed-sized buffer to replay past samples (rehearsal-based approach), regulating model parameter changes through learning (regularization-based approach), or dynamically expanding model architecture on demand (expansion-based approach). Among them, the rehearsal-based approach has shown great performance in continual learning settings, albeit with its simplicity. The idea of Experience Replay (ER \cite{riemer19}) is simply managing a fixed-sized buffer to retain a small number of samples and replaying those samples to prevent forgetting past knowledge. Following this simple setup, several methods have been proposed by expanding this framework in two aspects: which samples should be stored and how to utilize stored samples. 
Those works mainly focus on either regulating model updates not to contradict the learning objectives on past samples \cite{lopezpaz17, buzzega20} or selecting the most representative/forgetting-prone samples to prevent changes in past predictions \cite{aljundi19, chaudhry20, Rebuffi17}. In a purely decoupled representation learning setup, however, there are few studies on those two aspects since learning objectives of representation learning may not be directly aligned to the task-specific objectives in typical joint training schemes. In this work, we focus on utilizing buffered samples to learn representations continually on a decoupled representation-classifier learning scheme.
% Gradient based Sample Selection (GSS \cite{aljundi19}) formulates sample selection as a contrained optimization problem {\color{blue}that approximate the feasible region of original constraint from buffered samples.} Hindsight Anchor Learning (HAL \cite{chaudhry20}) attempts to {\color{blue}minimize forgetting while learning current task by approximating anchors that maximizes forgetting.} Gradient Episodic Memory (GEM \cite{lopezpaz17}) uses buffered samples to make sure that the current gradient update do not contradict the learning objective on past samples. iCaRL \cite{Rebuffi17} utilizes buffered samples to train the nearest-mean-of-exemplars classifier and distill learned representation for preventing representation from deteriorating. Dark Experience Knowledge Replay (DER \cite{buzzega20}) rehearses exemplars and its output logits to match current logit to past one to prevent forgetting. 

%\vspace{0.3em}
\noindent\textbf{Representation learning in continual learning.}
Only a few recent studies on continual learning focus on representations models learned in two aspects: how to maintain learned representations \cite{Rebuffi17} and how to learn representations accelerating future learning \cite{javed19, gupta20}. iCaRL \cite{Rebuffi17} prevents representations from being forgotten by leveraging distillation.
% while decoupling the concern of training classifier with the forgetting problem. 
% On the contrary, there also have been some studies that focus on training classifier with the belief that the changes in learned representation can be compensated by classifier training. However, the interest in representation itself in terms of preventing catastrophic forgetting has only recently begun to be studied.
Recent approaches \cite{javed19, gupta20} leverage meta-learning \cite{finn17} separate concerns of representation learning and classifier training and directly optimizes objectives that minimize forgetting by learning representations that accelerate future learning on meta-learning frameworks. 
% Look-ahead meta-learning (La-MAML\cite{gupta20}) extends such meta-learning based continual learning to be an online and scalable algorithm. 
% Those works learn such representations under decoupled representation-classifier training schemes but lack an explicit design to preserve representations. 
In this work, we focus on constructing representations that suffer less from forgetting and also focus on preserving learned representations in continual learning context not as a part of joint training. 
% Our work also focuses on continual representation learning under a similar philosophy, but we mainly leverage contrastive representation learning scheme based on our novel observation. 

%\vspace{0.5em}
\noindent\textbf{Contrastive representation learning.}
Recent progress in contrastive representation learning shows superior downstream task performance, even competitive to supervised training. Noise-contrastive estimation \cite{gutmann10} is the seminal work that estimates the latent distribution by contrasting with artificial noises. Info-NCE \cite{oord18} tries to learn representations from visual inputs by leveraging an auto-regressive model to predict the future in an unsupervised manner. Recent advances in this area stem from the use of multiple views as positive samples \cite{tian19}.
These core concepts have been followed by studies \cite{chen20, he20, grill2020bootstrap, chen2020exploring} that have resolved practical limitations that have previously made learning difficult such as negative sample pairs, large batch size, and momentum encoders. Meanwhile, it has been shown that supervised learning can also enjoy the benefits of contrastive representation learning by simply using labels to extend the definition of positive samples \cite{khosla20}. 
In this work, we mainly leverage contrastive representation learning schemes on the continual learning setup based on our novel observation (Section~\ref{subsection:observation}).

\vspace{0.2em}
\noindent\textbf{Knowledge distillation}. 
In continual learning, knowledge distillation is widely used to mitigate forgetting by distilling past signatures to the current models \cite{Li16, Rebuffi17}. However, it has not been studied to design/utilize knowledge distillation for decoupled representation-classifier training in the continual learning setup. In this work, we develop novel self-distillation loss for contrastive continual learning, which is inspired by the recently proposed distillation loss \cite{fang20} for contrastive learning framework.

% {\color{blue}In representation learning, Self-supervised distillation \cite{fang20} for contrastive representation learning framework has been recently proposed, which aims to distill contrastively trained model's representation to the smaller model.} In this work, we design distillation loss for contrastive continual learning, which is basically inspired by \cite{fang20}.

